Tensor Train for Global Optimization Problems in Robotics

The convergence of many numerical optimization techniques is highly dependent on the initial guess given to the solver. To address this issue, we propose a novel approach that utilizes tensor methods to initialize existing optimization solvers near global optima. Our method does not require access to a database of good solutions. We first transform the cost function, which depends on both task parameters and optimization variables, into a probability density function. Unlike existing approaches, the joint probability distribution of the task parameters and optimization variables is approximated using the Tensor Train model, which enables efficient conditioning and sampling. We treat the task parameters as random variables, and for a given task, we generate samples for decision variables from the conditional distribution to initialize the optimization solver. Our method can produce multiple solutions (when they exist) faster than existing methods. We first evaluate the approach on benchmark functions for numerical optimization that are hard to solve using gradient-based optimization solvers with a naive initialization. The results show that the proposed method can generate samples close to global optima and from multiple modes. We then demonstrate the generality and relevance of our framework to robotics by applying it to inverse kinematics with obstacles and motion planning problems with a 7-DoF manipulator.

==> sections/unused.tex <==

% \begin{table*}[!t]
%     \scriptsize 
%     \centering
% 	\renewcommand{\arraystretch}{1.3} % modify space between rows
% 	\setlength{\tabcolsep}{4pt}
% 	\caption{Performance for inverse kinematics of Panda}
% 	\begin{tabular}{@{\extracolsep{2pt}}ccc cccc cccc cccc cccc}
% 		\toprule[0.12em]
% 		\multirow{2}{*}{Method} & \multirow{2}{*}{$\alpha$} & \multicolumn{4}{c}{$\text{c}_\text{init}$} & \multicolumn{4}{c}{$\text{c}_\text{final}$} & \multicolumn{4}{c}{$\text{n}_\text{step}$} &  \multicolumn{4}{c}{\textbf{Success} (\%) }\\
% 		\cmidrule{3-6} \cmidrule{7-10} \cmidrule{11-14} \cmidrule{15-18}
% 		& & \#$1$ & \#$10$ & \#$100$ & \#$1000$ & \#$1$ & \#$10$ & \#$100$ & \#$1000$& \#$1$ & \#$10$ & \#$100$ & \#$1000$& \#$1$ & \#$10$ & \#$100$ & \#$1000$\\
% 		\midrule
% 		\multirow{5}{*}{TT Model} 
% 		& $0.99$ & $0$ &  $0$ & $0$ & $0$ &  $0$ & $0$ & $0$ &  $0$ & $0$ & $0$ &  $0$ & $0$ & $98$ &  $0$ & $0$ & $0$  \\
% 		& $0.9$ & $0$ & $0$ & $0$ & $0$ &  $0$ & $0$ & $0$ &  $0$ & $0$ & $0$ &  $0$ & $0$ & $0$ &  $0$ & $0$ & $0$ \\
% 		& $0.75$ & $0$ &  $0$ & $0$  & $0$ &  $0$ & $0$ & $0$ &  $0$ & $0$ & $0$ &  $0$ & $0$ & $0$ &  $0$ & $0$& $0$\\
% 		& $0.5$ & $0$ &  $0$ & $0$& $0$ &  $0$ & $0$ & $0$ &  $0$ & $0$ & $0$ &  $0$ & $0$ & $0$ &  $0$ & $0$ & $0$ 	\\
% 		& $0.$ & $0$ &  $0$ & $0$ & $0$ &  $0$ & $0$ & $0$ &  $0$ & $0$ & $0$ &  $0$ & $0$ & $0$ &  $0$ & $0$ & $0$   	\\
% 		\multirow{1}{*}{Uniform Distribution}
% 		& \- & $0$ & $0$ & $0$& $1.7$ & $0$& $0$ & $0$ & $0.17$& $0$ & $0$ & $0$ & $17.9$ & $63$& $75$ & $82$& $90$ \\
% %		
% %		\cmidrule{2-8}			
% %		\multirow{1}{*}{Uniform distribution} 
% %		& $-$ & $0$ &  $0$ & $0$ &  $0$ & $0$ &  $0$    \\
% %
% 		\bottomrule[0.12em]
% 	\end{tabular}
% 	\label{tab: ik_results}
% 	\vspace{-0.5cm}
% \end{table*}



% \begin{table*}
%     \centering
% 	\renewcommand{\arraystretch}{1.3} % modify space between rows
% 	\scriptsize
% 	\caption{Reaching two via-points in sequence}
% 	\begin{tabular}{ccc cccc cccc cccc cccc}
% 		\toprule[0.12em]
% 		\multirow{3}{*}{Method} & \multirow{3}{*}{$\alpha$} & \multicolumn{12}{c}{\textbf{\# Samples}} \\
% 		\cmidrule{3-14}
% 		& & \multicolumn{3}{c}{$1$} & \multicolumn{3}{c}{$100$} & \multicolumn{3}{c}{$1000$} &  \multicolumn{3}{c}{$10000$}\\
% 		\cmidrule{3-5} \cmidrule{6-8} \cmidrule{9-11} \cmidrule{12-14}
% 		& & $\text{c}_\text{i}$ & $\text{c}_\text{f}$  & \textbf{Success}  & $\text{c}_\text{i}$ & $\text{c}_\text{f}$ & \textbf{Success}  & $\text{c}_\text{i}$ & $\text{c}_\text{f}$ &  \textbf{Success} &  $\text{c}_\text{i}$ & $\text{c}_\text{f}$ & \textbf{Success} \\
% 		\midrule
% 		\multirow{4}{*}{TTGO} 
                		
%           & $0.9$ & $2.5$ & $0.18$ & $72.0$ & $1.08$ & $0.15$ & $82.0$ & $0.86$ & $0.15$ & $85.0$ & $0.71$ & $0.13$ & $89.0$ \\ & $0.75$ & $3.37$ & $0.16$ & $68.0$ & $1.31$ & $0.15$ & $77.0$ & $1.02$ & $0.14$ & $87.0$ & $0.83$ & $0.15$ & $81.0$ \\ & $0.5$ & $4.07$ & $0.21$ & $60.0$ & $1.6$ & $0.18$ & $76.0$ & $1.3$ & $0.16$ & $78.0$ & $1.04$ & $0.15$ & $87.0$ \\ & $0$ & $5.31$ & $0.29$ & $43.0$ & $2.14$ & $0.23$ & $60.0$ & $1.62$ & $0.15$ & $78.0$ & $1.3$ & $0.2$ & $72.0$ \\
% 		\cmidrule{3-6} \cmidrule{7-10} \cmidrule{11-14} \cmidrule{15-18}		
% 		\multirow{1}{*}{Uniform} 
%         &- & $9.34$ & $0.75$ & $27.5$ & $3.95$ & $0.45$ & $40.75$ & $3.07$ & $0.39$ & $41.5$ & $2.45$ & $0.33$ & $52.25$ \\ 
% 		\bottomrule[0.12em]
% 	\end{tabular}
% 	\label{tab: motion_via}
% 		\caption*{The performance measures for via points reaching task of Panda manipulator. The task is to reach two specified points in sequence: first point in the shelf (pick-up location)  and he second point on the box (drop location). The motion starts from a fixed initial configuration, reaches the two points in sequence and returns to the original configuration to complete a cycle. We compare the performance of TTGO for warm-starting the solver against random initialization. The three performance metrics are cost at the initialization ($c_i$), cost after fine-tuning ($c_f$) using a gradient-based optimizer (namely, SLQP) and the success rate. The criteria for success is that $c_f \leq 0.25$. We consider $100$ test cases containing pairs of target points in the shelf and on the box to compute the average of each of these measures. Each of the target points are chosen to be at least $8$cm away from the surface of the obstacle but they need not be accessible.}

% 		\caption*{The performance measures for target reaching of Panda manipulator. The task is to reach a specified point in the shelf from a fixed initial configuration. We compare the performance of TTGO for warm-starting the solver against random initialization. The three performance metrics are cost at the initialization ($c_i$), cost after fine-tuning ($c_f$) using a gradient-based optimizer (namely, SLQP) and the success rate. The criteria for success is that $c_f \leq 0.25$. We consider $100$ target points in the shelf and compute the average of each of these measures. Each of the target points are chosen to be at least $8$cm away from the surface of the obstacle but they need not be accessible.}






